On Over-Squashing in Message Passing Neural Networks: The Impact of Width, Depth, and Topology

Message Passing Neural Networks (MPNNs) are instances of Graph Neural Networks that leverage the graph to send messages over the edges. This inductive bias leads to a phenomenon known as over-squashing, where a node feature is insensitive to information contained at distant nodes. Despite recent methods introduced to mitigate this issue, an understanding of the causes for over-squashing and of possible solutions are lacking. In this theoretical work, we prove that: (i) Neural network width can mitigate over-squashing, but at the cost of making the whole network more sensitive; (ii) Conversely, depth cannot help mitigate over-squashing: increasing the number of layers leads to over-squashing being dominated by vanishing gradients; (iii) The graph topology plays the greatest role, since over-squashing occurs between nodes at high commute (access) time. Our analysis provides a unified framework to study different recent methods introduced to cope with over-squashing and serves as a justification for a class of methods that fall under graph rewiring.

==> commands.tex <==
\definecolor{ggblue}{RGB}{36, 100, 137} 
\definecolor{ggred}{RGB}{226, 74, 51}
\definecolor{ggpurple}{RGB}{95,87,145}

\hypersetup{
    colorlinks = true,
    citecolor = {ggpurple},
    urlcolor = {ggblue},
    linkcolor = {ggred}
}
\usepackage{url}


==> sections/walk_importance.tex <==
\section{How to Escape Labyrinths}
In graph representation learning, the term \emph{"long range interaction"} often refers to an unknown function $f(\mathbf{x}_i, \mathbf{x}_j)$ which takes the feature vectors of two nodes $i$ and $j$ that are several hops away from each other and provides meaningful insights for the learning task. 

Capture those interactions is still an unsolved problem since in the plethora of methods available in literature, the information is accumulated breath-wise which leads to the well known  problems in graph neural networks (i.e. oversmoothing and oversquashing). In particular, in heterophilic settings, capture those interactions become essential since, by definition, looking to the first-order neighbourhoods leads to aggregate misleading information  w.r.t. the classification task.


Considering that  the $i$-th row of $\bar{A}^k$ contains the number of \emph{walks} of length $k$ from node $i$ to the rest of the graph normalized by their degrees, we might propagate the information contained in a node $i$ to its k-hop neighbours using the powers of the normalized adjacency matrix.

However, for some nodes with high clustering coefficient, the direct spatial diffusion process in Equation (\ref{eq:power_series}) might prevent a signal to reach remote parts of the graph, making it bounce within a local neighbourhood of the node itself (mirroring). To avoid the mirroring effect, we have to design a \emph{correction} tensor $\bar{S}$ such that:

\begin{equation}
    [\bar{S}_k]_{i,j} = 
    \begin{cases} 
      c \cdot d(i,j) & \text{if $j$ is reachable from $i$ in $k$ hops}\\
      0 & \text{otherwise}
   \end{cases}
\end{equation}

for some real constant $c$, and $d(i,j)$ to be the distance between $i$ and $j$. To do so, we set $\bar{S}_k = -\log(\Gamma_k \odot \bar{A}^k)$, where $\Gamma_k$ is a matrix constant on the columns and the rows are defined as follows:

\begin{equation}
    [\Gamma_k]_i = lse\left([\bar{A}^k]_i\right) = \max\left([\bar{A}^k]_i\right) + \log\left( \sum_j \exp\left([\bar{A}^k]_{i,j} - \max\left([\bar{A}^k]_i\right) \right) \right)
\end{equation}



in Equation (\ref{eq:signal_diffusion}) highlights the information provided by the nodes that are not yet visited in the walks of length $k' : 0 \leq k' < k$.





if $\mathbf{X} \in \mathbb{R}^{N \times d}$ is the feature matrix associated to the nodes of the graph we have that the $i$-th row of  $\bar{A}^k \mathbf{X}$ 



In this section we want to provide an intuition on how to compute the importance of a walk $\gamma(i,j; m)$, from a node $i$ to a node $j$ of length $m$.

Recall that $\boldsymbol{\omega}(i;m) = [\bar{A}^m]_i$ provides the number of \emph{walks} of length $m$ starting from node $i$, normalized by the respective nodes' degrees. 

Collecting all the values $\gamma(i,j; m)$ into a tensor $\Gamma \in \mathbb{R}^{N\times N\times M}$ and stacking all the adjacencies $A^m$ into a tensor $\mathbb{A}^{N\times N\times M}$ we have that the forward pass for a feature matrix $\mathbf{X} \in \mathbb{R}^{N \times F}$ is provided by:

\begin{align}
    \mathbf{\Tilde{X}} &= enc(\mathbf{X})  \in \mathbb{R}^{N \times F'}  \\
    \mathbf{Z} &= \sum_m \underbrace{\Gamma_m \odot \mathbb{\bar{A}}_m}_{\zeta_m} \mathbf{\Tilde{X}} \mathbf{W}_m
\end{align}

In practice, $\zeta_m$ highlights the information provided by the nodes that are not yet visited in the walks of length $m' : 0 \leq m' < m$. To do so, we set $\boldsymbol{\gamma}(i; m) = \frac{1}{lse(\boldsymbol{\omega}(i;m))}$, where $lse(\boldsymbol{\omega}(i;m)) = \max{(\boldsymbol{\omega}(i;m))} + \log{(\sum_j \exp{(x_j - \max{(\boldsymbol{\omega}(i;m))})})}$  \cite{nielsen2016guaranteed}

